On random embeddings and their application to optimisation

Random embeddings project high-dimensional spaces to low-dimensional ones; they are careful constructions which allow the approximate preservation of key properties, such as the pair-wise distances between points. Often in the field of optimisation, one needs to explore high-dimensional spaces representing the problem data or its parameters and thus the computational cost of solving an optimisation problem is connected to the size of the data/variables. This thesis studies the theoretical properties of norm-preserving random embeddings, and their application to several classes of optimisation problems.

==> Tex/1._Intro/4._Related_literature.tex <==
The key technique used in this thesis is the random embedding, which is introduced in detail in the beginning of the next Chapter. Here we separately review the relevant recent advances of solving \eqref{LLS-statement} and \eqref{general_objective_statement}.

\subsection{Recent advances in solving \eqref{LLS-statement}}

\paragraph{Short Summary}










==> Tex/4._First_order_subspace_methods/6._numerics.tex <==
In this section, we will numerically test R-SGN with trust-region using different choices of the sketching matrix $S_k$ (results for quadratic regularisation are comparable and given in the appendix). We will use suitable subsets of the extensive CUTEst test collection \cite{gould2015cutest}. We will measure performance using data profiles, a variant of performance profiles \cite{dolan2002benchmarking}, over Jacobian actions and runtime. That is, for each solver $s$, each test problem $p \in \mathcal{P}$ and for an accuracy level $\tau\in(0,1)$, we determine the number of Jacobian action evaluations $N_p(s,\tau)$ required for a problem to be solved: \todo{Define Jacobian action evalutations.}
\[
N_p(s,\tau) \deq \text{no.\ Jacobian action evaluations required until } f(x_k) \le f^* + \tau(f(x_0) - f^*), 
\]
where $f^*$ is an estimate of the true minimum $f(x^*)$. (Note that sometimes $f^*$ is taken to be the best value achieved by any solver.) We define $N_p(s,\tau)=\infty$ if this was not achieved in the maximum computational budget allowed, which we take to be $50d_p$ Jacobian action evaluations where $d_p$ is the dimension of test problem $p$.
To obtain data profiles, we can then normalise $N_p(s,\tau)$ by the problem dimension $d_p$. That is, we plot
\[
\pi_{s,\tau}^N(\alpha) \deq \frac{\abs{\{p\in\mathcal{P} : N_p(s,\tau) \le \alpha 
d_p\}}}{\abs{\mathcal{P}}}, \qquad \text{for } \alpha \in [0,50].
\]
We perform $100$ runs of each R-SGN variant (since R-SGN is a randomised algorithm) and thus to enable fair comparison, we treat each run as a separate `problem' in the above.

\subsection{Zero residual CUTEst problems}
First we will consider a test set of 32 zero-residual ($f(x^*)=0$) nonlinear least squares problems from CUTEst, given in \autoref{tab:cutest32}. These problems mostly have dimension around $d=100$, although one or two have $d=50$ to $64$. Our reasons for choosing $d\approx100$ are twofold: firstly this gives us a large test set of problems, secondly we can perform 100 random runs of R-SGN in reasonable time for all 32 problems.  
Since we are primarily interested in R-SGN performance in the low-accuracy setting, we will set the accuracy level $\tau=10^{-1}$ when calculating the data profiles. 

\begin{table}[!h]
\centering
\begin{tabular}{lrrlrrlrr}  
\toprule
Name & $d$ & $n$ & Name & $d$ & $n$ & Name & $d$ & $n$ \\
\midrule
ARGTRIG & 100 & 100 & DRCAVTY1 & 100 & 100 & OSCIGRNE & 100 & 100 \\
ARTIF & 100 & 100 & DRCAVTY3 & 100 & 100 & POWELLSE & 100 & 100 \\
BDVALUES & 100 & 100 & EIGENA & 110 & 110 & SEMICN2U & 100 & 100 \\
BRATU2D & 64 & 64 & EIGENB & 110 & 110 & SEMICON2 & 100 & 100 \\
BROWNALE & 100 & 100 & FLOSP2TL & 59 & 59 & SPMSQRT & 100 & 164 \\
BROYDN3D & 100 & 100 & FLOSP2TM & 59 & 59 & VARDIMNE & 100 & 102 \\
BROYDNBD & 100 & 100 & HYDCAR20 & 99 & 99 & LUKSAN11 & 100 & 198 \\
CBRATU2D & 50 & 50 & INTEGREQ & 100 & 100 & LUKSAN21 & 100 & 100 \\
CHANDHEQ & 100 & 100 & MOREBVNE & 100 & 100 & YATP1NE & 120 & 120 \\
CHEMRCTA & 100 & 100 & MSQRTA & 100 & 100 & YATP2SQ & 120 & 120 \\
CHNRSBNE & 50 & 98 & MSQRTB & 100 & 100 & & & \\
\bottomrule
\end{tabular}
\caption{The 32 CUTEst test problems in the zero-residual test set.}\label{tab:cutest32}
\end{table}

Let us start by looking at the performance of R-SGN with coordinate sampling matrices $S_k$. \highlight{Or scaled sampling?} In \autoref{fig:cutest32_coordinate}, we can see the Jacobian action evaluations data profile and clearly Gauss-Newton is superior from a Jacobian action budget perspective.
Next, we compare the performance of R-SGN with Gaussian sketching matrices $S_k$. In \autoref{fig:cutest32_gaussian}, we can see the Jacobian action evaluations data profile and once again, we see that Gauss-Newton is better from a Jacobian action budget perspective.
Finally, we compare the performance of R-SGN with 3-hashing sketching matrices $S_k$. In \autoref{fig:cutest32_hashing}, we can see the Jacobian action evaluations data profile, once again, we see that Gauss-Newton is clearly superior from a Jacobian action budget perspective. 
It is also useful to compare across the different sketching matrices and to this end we plot the Jacobian actions data profile for a subspace size of $0.75d$ in \autoref{fig:cutest32_across}. We see from the figure that interestingly sampling matrices exhibit the best performance from a Jacobian action budget perspective.

\begin{figure}[!p]
\centering
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst32 Fixed/coordinate/BCGN-TR-NORMAL-COORDINATE-1e-01_coordevals.png}
\caption{R-SGN data profiles on the zero-residual test set with coordinate sampling for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest32_coordinate}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst32 Fixed/gaussian/BCGN-TR-NORMAL-GAUSSIAN-1e-01_coordevals.png}
\caption{R-SGN data profiles on the zero-residual test set with Gaussian sketching for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest32_gaussian}
\end{minipage}
\end{figure}

\begin{figure}[!p]
\centering
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst32 Fixed/hashing/BCGN-TR-NORMAL-HASHING-1e-01_coordevals.png}
\caption{R-SGN data profiles on the zero-residual test set with $3$-hashing sketching for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest32_hashing}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst32 Fixed/across/BCGN-TR-NORMAL-1e-01_coordevals.png}
\caption{R-SGN data profiles on the zero-residual test set with the various sketching matrices for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest32_across}
\end{minipage}
\end{figure}

\subsection{Nonzero residual CUTEst problems}
Next, we consider a test set of 19 nonzero-residual ($f(x^*)\neq 0$) nonlinear least squares problems from CUTEst, given in \autoref{tab:cutest19}. As before, these problems mostly have dimension around $d=100$ with a few having $d=59$ to $64$, for reasons previously discussed. We will also set the accuracy level $\tau=10^{-1}$ as before. 

\begin{table}[!h]
\centering
\begin{tabular}{lrrlrrlrr}  
\toprule
Name & $d$ & $n$ & Name & $d$ & $n$ & Name & $d$ & $n$ \\
\midrule
ARGLALE & 100 & 400 & FLOSP2HL & 59 & 59 & LUKSAN14 & 98 & 224 \\
ARGLBLE & 100 & 400 & FLOSP2HM & 59 & 59 & LUKSAN15 & 100 & 196 \\
ARWHDNE & 100 & 198 & FREURONE & 100 & 198 & LUKSAN16 & 100 & 196 \\
BRATU2DT & 64 & 64 & PENLT1NE & 100 & 101 & LUKSAN17 & 100 & 196 \\
CHEMRCTB & 100 & 100 & PENLT12NE & 100 & 200 & LUKSAN22 & 100 & 198 \\
DRCAVTY2 & 100 & 100 & LUKSAN12 & 98 & 192 & & & \\
FLOSP2HH & 59 & 59 & LUKSAN13 & 98 & 224 & & & \\
\bottomrule
\end{tabular}
\caption{The 19 CUTEst test problems in the nonzero-residual test set.}\label{tab:cutest19}
\end{table}

Let us start by looking at the performance of R-SGN with coordinate sampling matrices $S_k$. In \autoref{fig:cutest19_coordinate}, we can see the Jacobian action evaluations data profile and we see that Gauss-Newton is clearly superior from a Jacobian action budget perspective. 
Next, we compare the performance of R-SGN with Gaussian sketching matrices $S_k$. In \autoref{fig:cutest19_gaussian}, we can see the Jacobian action evaluations data profile and as before, we continue to see the superiority of Gauss-Newton from a Jacobian action budget perspective.
Finally, we compare the performance of R-SGN with 3-hashing sketching matrices $S_k$. In \autoref{fig:cutest19_hashing}, we can see the Jacobian action evaluations data and unsurprisingly, we again see the superiority of Gauss-Newton from a Jacobian action budget perspective.
It is also useful to compare across the different sketching matrices and to this end we plot the Jacobian actions data profile for a subspace size of $0.75d$ in \autoref{fig:cutest19_across}. We see from the figure that once again sampling matrices exhibit the best performance from a Jacobian action budget perspective.

\begin{figure}[!p]
\centering
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst Nonzero Fixed/coordinate/BCGN-TR-NORMAL-COORDINATE-1e-01_coordevals.png}
\caption{R-SGN data profiles on the nonzero-residual test set with coordinate sampling for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest19_coordinate}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst Nonzero Fixed/gaussian/BCGN-TR-NORMAL-GAUSSIAN-1e-01_coordevals.png}
\caption{R-SGN data profiles on the nonzero-residual test with Gaussian sketching for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest19_gaussian}
\end{minipage}
\end{figure}

\begin{figure}[!p]
\centering
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst Nonzero Fixed/hashing/BCGN-TR-NORMAL-HASHING-1e-01_coordevals.png}
\caption{R-SGN data profiles on the nonzero-residual test set with $3$-hashing sketching for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest19_hashing}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
\includegraphics[width=\textwidth]{images/BCGN_Figures/CUTEst Nonzero Fixed/across/BCGN-TR-NORMAL-1e-01_coordevals.png}
\caption{R-SGN data profiles on the nonzero-residual test set with the various sketching matrices for an accuracy of $\tau=10^{-1}$.}
\label{fig:cutest19_across}
\end{minipage}
\end{figure}

\subsection{Large-scale CUTEst problems}
In this section we will look at the behaviour of R-SGN on three large-scale ($d\approx5,000$ to $10,000$) problems from the CUTEst collection. The three problems are given in \autoref{tab:cutestind}. As the dimension of the problems is so large and we would like individual insight into each problem, we will only run R-SGN five times on each problem until we achieve a $10^{-1}$ decrease in the objective, or failing that, for a maximum of 20 iterations. Furthermore, we will not use data profiles but rather plot the objective decrease against cumulative Jacobian action evaluations for each random run with block-sizes of 1\%, 5\%, 10\%, 50\%, 100\% of the original. 

\begin{table}[!h]
\centering
\begin{tabular}{lrrlrrlrr}  
\toprule
Name & $d$ & $n$ & Name & $d$ & $n$ & Name & $d$ & $n$ \\
\midrule
ARTIF & 5,000 & 5,000 & BRATU2D & 4,900 & 4,900 & OSCIGRNE & 10,000 & 10,000 \\
\bottomrule
\end{tabular}
\caption{The 3 large-scale CUTEst test problems.}\label{tab:cutestind}
\end{table}

Let us start by looking at the performance of R-SGN with coordinate sampling matrices $S_k$. In \autoref{fig:large_coordinate}, we can see the objective decrease against cumulative Jacobian action evaluations for ARTIF, BRATU2D and OSCIGRNE. On ARTIF, we see that while R-SGN exhibits comparable performance, Gauss-Newton is clearly superior from a Jacobian action budget perspective. On BRATU2D we see that R-SGN really struggles to achieve any meaningful decrease, as does Gauss-Newton initially but then switches to a quadratic regime and quickly converges. On OSCIGRNE, we see that R-SGN with subspace sizes of $0.05d,0.1d,0.5d$ sometimes performs very well (outperforming Gauss-Newton) but sometimes struggles, and on averages Gauss-Newton performs better.

Next, we compare the performance of R-SGN with Gaussian sketching matrices $S_k$. In \autoref{fig:large_gaussian}, we can see the objective decrease against cumulative Jacobian action evaluations for ARTIF, BRATU2D and OSCIGRNE. On ARTIF, we see that R-SGN with a subspace size of $0.5d$ outperforms Gauss-Newton initially before stagnating. On BRATU2D we once again see that R-SGN struggles to achieve any meaningful decrease, as does Gauss-Newton initially but then switches to a quadratic regime and quickly converges. However, on OSCIGRNE we see that R-SGN with a subspace size of $0.5d$ consistently outperforms Gauss-Newton.

Finally, we compare the performance of R-SGN with 3-hashing sketching matrices $S_k$. In \autoref{fig:large_hashing}, we can see the objective decrease against cumulative Jacobian action evaluations for ARTIF, BRATU2D and OSCIGRNE. On ARTIF, we again see that R-SGN with a subspace size of $0.5d$ outperforms Gauss-Newton initially before stagnating. On BRATU2D we once again see that R-SGN struggles to achieve any meaningful decrease, as does Gauss-Newton initially but then switches to a quadratic regime and quickly converges. However, on OSCIGRNE we again see that R-SGN with a subspace size of $0.5d$ consistently outperforms Gauss-Newton. 

% COORDINATE
\begin{figure}[!h]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/coordinate/ARTIF_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/coordinate/BRATU2D_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/coordinate/OSCIGRNE_blocks.png}
\end{subfigure}
\caption{ARTIF (left), BRATU2D (middle) and OSCIGRNE (right) objective value against cumulative Jacobian action size for R-SGN with coordinate sampling.}
\label{fig:large_coordinate}
\end{figure}

%It may be hard to see from the figure, but R-SGN on BRATU2D is actually converging albeit extermely slowly, as can be seen from the following close up in \autoref{fig:bratu2d_coord_zoom}.
%\begin{figure}[!h]
%\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/coordinate/BRATU2D_zoom.png}
%\caption{Close up zoom of very slow R-SGN convergence on BRATU2D.}
%\label{fig:bratu2d_coord_zoom}
%\end{figure}

% GAUSSIAN
\begin{figure}[!h]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/gaussian/ARTIF_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/gaussian/BRATU2D_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/gaussian/OSCIGRNE_blocks.png}
\end{subfigure}
\caption{ARTIF (left), BRATU2D (middle) and OSCIGRNE (right) objective value against cumulative Jacobian action size for R-SGN with Gaussian sketching.}
\label{fig:large_gaussian}
\end{figure}

%It may be hard to see from the figure, but R-SGN on BRATU2D is actually converging albeit extermely slowly, as can be seen from the following close up in \autoref{fig:bratu2d_gauss_zoom}.
%\begin{figure}[!h]
%\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/gaussian/BRATU2D_zoom.png}
%\caption{Close up zoom of very slow R-SGN convergence on BRATU2D.}
%\label{fig:bratu2d_gauss_zoom}
%\end{figure}

% HASHING
\begin{figure}[!h]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/hashing/ARTIF_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/hashing/BRATU2D_blocks.png}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/hashing/OSCIGRNE_blocks.png}
\end{subfigure}
\caption{ARTIF (left), BRATU2D (middle) and OSCIGRNE (right) objective value against cumulative Jacobian action size for R-SGN with $3$-hashing sketching.}
\label{fig:large_hashing}
\end{figure}

%It may be hard to see from the figure, but R-SGN on BRATU2D is actually converging albeit extermely slowly, as can be seen from the following close up in \autoref{fig:bratu2d_hash_zoom}.
%\begin{figure}[!h]
%\includegraphics[width=\textwidth]{images/BCGN_Figures/Individual/hashing/BRATU2D_zoom.png}
%\caption{Close up zoom of very slow R-SGN convergence on BRATU2D.}
%\label{fig:bratu2d_hash_zoom}
%\end{figure}

%% ADAPTIVE BRATU2D
\subsection{Adaptive R-SGN}
Finally, we highlight a variant of R-SGN where we adaptively increase the subspace size. Starting from a fixed dimensional subspace, we adaptively increase the subspace by a fixed amount until we achieve sufficient decrease in the quadratic model, i.e.\ until
\[
q_k(s_k) \le \kappa q_k(0)
\]
where $s_k$ is the $k$-th regularisation or trust region step and $\kappa\in(0,1)$ is our adaptivity parameter (note that $\kappa=1$ corresponds to using the full dimensional space, i.e.\ Gauss-Newton in the case of sampling). 

%% COORDINATE
% BRATU2D
\begin{figure}[!h]
\centering
\includegraphics[width=0.5\textwidth]{images/BCGN_Figures/Indiv_adap/coordinate/BRATU2D_blocks.png}
\caption{BRATU2D objective value against cumulative Jacobian action size for Adaptive R-SGN with coordinate sampling starting at the subspace sizes indicated.}
\label{fig:bratu2d_adaptive}
\end{figure}

In \autoref{fig:bratu2d_adaptive} we show adaptive R-SGN with coordinate sampling for the BRATU2D test problem, starting at the subspace sizes indicated in the figure and the increasing by increments of $500$.  

